MSPM: A Multi-Site Physiological Monitoring Dataset for Remote Pulse, Respiration, and Blood Pressure Estimation

Visible-light cameras can capture subtle physiological biomarkers without physical contact with the subject. We present the Multi-Site Physiological Monitoring (MSPM) dataset, which is the first dataset collected to support the study of simultaneous camera-based vital signs estimation from multiple locations on the body. MSPM enables research on remote photoplethysmography (rPPG), respiration rate, and pulse transit time (PTT); it contains ground-truth measurements of pulse oximetry (at multiple body locations) and blood pressure using contacting sensors. We provide thorough experiments demonstrating the suitability of MSPM to support research on rPPG, respiration rate, and PTT. Cross-dataset rPPG experiments reveal that MSPM is a challenging yet high quality dataset, with intra-dataset pulse rate mean absolute error (MAE) below 4 beats per minute (BPM), and cross-dataset pulse rate MAE below 2 BPM in certain cases. Respiration experiments find a MAE of 1.09 breaths per minute by extracting motion features from the chest. PTT experiments find that across the pairs of different body sites, there is high correlation between remote PTT and contact-measured PTT, which facilitates the possibility for future camera-based PTT research.

==> tables/old/all2mspm.tex <==

\begin{table}[]
    \centering
    \begin{tabular}{cc|cc}
        \toprule
        Train Dataset & Portion      & MAE                & MXCorr            \\
        \midrule
        %DDPM & mcc        & 9.656 $\pm$ 3.889  & 0.562 $\pm$ 0.045 \\
        %DDPM & negpearson & 8.212 $\pm$ 0.225  & 0.612 $\pm$ 0.016 \\
        DDPM & full & 8.212 $\pm$ 0.225  & 0.612 $\pm$ 0.016 \\
        DDPM & attack & 37.060 $\pm$ 0.303 & 0.172 $\pm$ 0.011 \\
        DDPM & not attack & 2.696 $\pm$ 0.203  & 0.697 $\pm$ 0.019 \\
        \midrule
        %PURE & mcc        & 14.832 $\pm$ 2.772 & 0.382 $\pm$ 0.081 \\
        %PURE & negpearson & 14.912 $\pm$ 3.610 & 0.363 $\pm$ 0.109 \\
        PURE & full & 14.912 $\pm$ 3.610 & 0.363 $\pm$ 0.109 \\
        PURE & attack & 38.385 $\pm$ 1.317 & 0.151 $\pm$ 0.045 \\
        PURE & not attack & 10.297 $\pm$ 4.150 & 0.409 $\pm$ 0.122 \\
        \midrule
        %UBFC & mcc        & 13.839 $\pm$ 4.393 & 0.437 $\pm$ 0.066 \\
        %UBFC & negpearson & 11.912 $\pm$ 4.748 & 0.484 $\pm$ 0.116 \\
        UBFC & full & 11.912 $\pm$ 4.748 & 0.484 $\pm$ 0.116 \\
        \bottomrule
    \end{tabular}
    \caption{Cross-dataset results for training on DDPM, PURE, and UBFC, and evaluating on MSPM.}
    \label{tab:all2mspm}
\end{table}

==> tables/old/intra-dataset-old.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{cc|cc}
        \toprule
        Dataset & Loss & MAE & MXCorr \\
        \midrule
        MSPM & negpearson & 7.147 $\pm$ 1.043 & 0.665 $\pm$ 0.093 \\
        MSPM & mcc        & 2.431 $\pm$ 1.016 & 0.754 $\pm$ 0.099 \\
        MSPM & negp.+mcc & 4.245 $\pm$ 0.902 & 0.723 $\pm$ 0.096 \\
        \midrule
        DDPM & negpearson & 2.492 $\pm$ 2.171 & 0.566 $\pm$ 0.082 \\
        DDPM & mcc        & 2.968 $\pm$ 1.824 & 0.559 $\pm$ 0.073 \\
        \midrule
        PURE & negpearson & 0.814 $\pm$ 0.676 & 0.730 $\pm$ 0.090 \\
        PURE & mcc        & 0.858 $\pm$ 1.032 & 0.752 $\pm$ 0.098 \\
        \midrule
        UBFC & negpearson & 0.935 $\pm$ 0.587 & 0.767 $\pm$ 0.028 \\
        UBFC & mcc        & 1.368 $\pm$ 1.150 & 0.748 $\pm$ 0.054 \\
        \bottomrule
    \end{tabular}
    \caption{Intra-dataset results for MSPM, DDPM, PURE, and UBFC.}
    \label{tab:all_intra}
\end{table}

==> tables/old/mspm-breakdown-old.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{cc|cc}
        \toprule
        Portion & Loss & MAE & MXCorr \\
        \midrule
        full & negpearson        & 7.147 $\pm$ 1.043  & 0.665 $\pm$ 0.093 \\
        full & mcc  & 2.431 $\pm$ 1.016 & 0.754 $\pm$ 0.099 \\
        full & negp.+mcc & 4.245 $\pm$ 0.902  & 0.723 $\pm$ 0.096 \\
        \midrule
        relaxed & negpearson     & 1.812 $\pm$ 0.737  & 0.718 $\pm$ 0.095 \\
        relaxed & mcc  & 1.210 $\pm$ 0.478 & 0.784 $\pm$ 0.088 \\
        relaxed & negp.+mcc & 1.370 $\pm$ 0.524  & 0.753 $\pm$ 0.096 \\
        \midrule
        game & negpearson       & 2.026 $\pm$ 1.182  & 0.804 $\pm$ 0.074 \\
        game & mcc & 1.560 $\pm$ 1.138 & 0.884 $\pm$ 0.063 \\
        game & negp.+mcc & 1.782 $\pm$ 1.227  & 0.850 $\pm$ 0.064 \\
        \midrule
        breath hold & negpearson & 1.992 $\pm$ 0.824  & 0.809 $\pm$ 0.060 \\
        breath hold & mcc & 1.577 $\pm$ 0.691 & 0.878 $\pm$ 0.050 \\
        breath hold & negp.+mcc & 1.817 $\pm$ 0.682  & 0.846 $\pm$ 0.053 \\
        \midrule
        BW video & negpearson    & 2.658 $\pm$ 3.525  & 0.822 $\pm$ 0.095 \\
        BW video & mcc & 2.160 $\pm$ 3.576 & 0.891 $\pm$ 0.072 \\
        BW video & negp.+mcc & 2.309 $\pm$ 3.586  & 0.869 $\pm$ 0.071 \\
        \midrule
        RGB video & negpearson  & 1.643 $\pm$ 1.162  & 0.835 $\pm$ 0.047 \\
        RGB video & mcc & 1.275 $\pm$ 1.377 & 0.902 $\pm$ 0.036 \\
        RGB video & negp.+mcc & 1.335 $\pm$ 1.377  & 0.877 $\pm$ 0.040 \\
        \midrule
        attack & negpearson     & 35.750 $\pm$ 1.951 & 0.280 $\pm$ 0.035 \\
        attack & mcc & 8.011 $\pm$ 2.218 & 0.698 $\pm$ 0.103 \\
        attack & negp.+mcc & 18.715 $\pm$ 7.235 & 0.554 $\pm$ 0.112 \\
        \bottomrule
    \end{tabular}
    \caption{Intra-dataset breakdown of results for MSPM by session portion.}
    \label{tab:mspm_intra}
\end{table}

==> tables/old/mspm2all.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{cc|cc}
        \toprule
        Test Dataset & Loss      & MAE                 & MXCorr            \\
        \midrule
        DDPM & mcc        & 20.259 $\pm$ 4.172  & 0.330 $\pm$ 0.044 \\
        DDPM & negpearson & 25.574 $\pm$ 3.213  & 0.235 $\pm$ 0.020 \\
        DDPM & negp.+mcc & 21.830 $\pm$ 4.574  & 0.278 $\pm$ 0.037 \\
        \midrule
        PURE & mcc        & 23.993 $\pm$ 25.203 & 0.356 $\pm$ 0.141 \\
        PURE & negpearson & 5.717 $\pm$ 1.314   & 0.501 $\pm$ 0.045 \\
        PURE & negp.+mcc & 12.440 $\pm$ 6.469  & 0.396 $\pm$ 0.106 \\
        \midrule
        UBFC & mcc        & 21.149 $\pm$ 14.914 & 0.340 $\pm$ 0.200 \\
        UBFC & negpearson & 9.459 $\pm$ 11.497  & 0.520 $\pm$ 0.213 \\
        UBFC & negp.+mcc & 18.081 $\pm$ 10.122 & 0.368 $\pm$ 0.157 \\
        \bottomrule
    \end{tabular}
    \caption{Cross-dataset results for training on MSPM and evaluating on DDPM, PURE, and UBFC.}
    \label{tab:mspm2all}
\end{table}
